Who is Undercover? Guiding LLMs to Explore Multi-Perspective Team Tactic in the Game

Large Language Models (LLMs) are pivotal AI agents in complex tasks but still face challenges in open decision-making problems within complex scenarios. To address this, we use the language logic game ``Who is Undercover?'' (WIU) as an experimental platform to propose the Multi-Perspective Team Tactic (MPTT) framework. MPTT aims to cultivate LLMs' human-like language expression logic, multi-dimensional thinking, and self-perception in complex scenarios. By alternating speaking and voting sessions, integrating techniques like self-perspective, identity-determination, self-reflection, self-summary and multi-round find-teammates, LLM agents make rational decisions through strategic concealment and communication, fostering human-like trust. Preliminary results show that MPTT, combined with WIU, leverages LLMs' cognitive capabilities to create a decision-making framework that can simulate real society. This framework aids minority groups in communication and expression, promoting fairness and diversity in decision-making. Additionally, our Human-in-the-loop experiments demonstrate that LLMs can learn and align with human behaviors through interactive, indicating their potential for active participation in societal decision-making.

==> sections/gaming.tex <==

\section{Game description and role settings}
"Who is Undercover?" (WIU) is a reasoning game where five players are randomly assigned the roles of either civilians (3) or undercovers (2). Each player receives a word that they must describe in short sentences, highlighting common features while concealing their specific word. Players must judge their roles and subtly signal to teammates without repeating others' speeches. Voting occurs at the end of each round, aiming to eliminate opposing players. If all undercovers remain undiscovered until only one civilian is left, the undercovers win; otherwise, the civilians win. The challenge lies in discerning one's role as the words have many similarities.



